Synthesize, Execute and Debug: Learning to Repair for Neural Program Synthesis

The use of deep learning techniques has achieved significant progress for program synthesis from input-output examples. However, when the program semantics become more complex, it still remains a challenge to synthesize programs that are consistent with the specification. In this work, we propose SED, a neural program generation framework that incorporates synthesis, execution, and debugging stages. Instead of purely relying on the neural program synthesizer to generate the final program, SED first produces initial programs using the neural program synthesizer component, then utilizes a neural program debugger to iteratively repair the generated programs. The integration of the debugger component enables SED to modify the programs based on the execution results and specification, which resembles the coding process of human programmers. On Karel, a challenging input-output program synthesis benchmark, SED reduces the error rate of the neural program synthesizer itself by a considerable margin, and outperforms the standard beam search for decoding.

==> backup.tex <==
Program synthesis has focused on synthesizing programs from some human provided specification, while program repair has focused on fixing human-introduced errors in programs, with the goal of debugging automatically human generated programs. 

However, for humans, the synthesis and repair are not separate tasks, but rather program repair is part of the process of synthesis, in which a program is repeatedly edited until the designer is satisfied in the result. This is often accomplished for sequential programming tasks by the use of a REPL in which parts of the program can be executed and their results analyzed, which has inspired work in program synthesis. \cite{Ellis2019WriteEAExtendExecution} However, for programs that are loop-containing, a REPL is not the usual mode in which humans adjust their programs. Instead, they typically \emph{debug} their programs by running a completed program against some test case and observing its behavior to see what needs to be changed. Our SED model similarly first synthesizes and then iteratively improves the program in order to find programs for examples that would be difficult to find in one shot.

Precisely, there is some latent prior on programs $P(p)$ and on program inputs $P(x | p)$. The prior is such that $p(x)$ is always defined when $x \sim P(x | p)$. The neural synthesizer is a model $M$ that is given input/output examples $(x_1, p(x_1)), \ldots, (x_k, p(x_k))$ where $p \sim P(p)$ and $x_k \sim P(x | p)$ and produces a program $p^\star$. $p^\star$ is considered correct if $p^\star(x) = p(x)$ for $x \in \{x_1 \ldots x_k\}$ and $p^\star(x_{k + 1}) = p(x_{k + 1})$, where $x_{k + 1} \sim P(i | p)$ is drawn independently of each of the other inputs.

 In a sense, this problem can be viewed as a generalization of the regression problem, in which there is some dataset $(x, y) \sim D$ and the model $M$ is given training input/output examples $(x, y) \sim D$, and its goal is to create a function that can match independently drawn evaluation samples $(x, y) \sim D$. For example, in linear regression, the model $M$ takes in $(x_1, y_1) \ldots (x_k, y_k)$ and returns a weights vector $w$ that represents the program $x \mapsto w^T x$, which best matches the given data.
 
 Figure~\ref{fig:arch_fine} shows a comparison of architectures and finetuning results for each model. One clear factor is that editing steps appear to have a roughly logarithmic relationship with error, with error reducing roughly linearly in the $\log$ of the number of editing steps. The improvement begins to converge as the number of steps rises above 10-25, and seems to converge more quickly for unfinetuned models. Additionally, we see the same patterns as from table~\ref{tab:main-results}, in which finetuning seems to have a fairly large effect on the results when using LGRL-GD and LGRL synthesizers, and TraceEmbed mostly seems to produce benefits when finetuning is not also used, but only in LGRL and EGNPS.
 
 We find that it is able to combine a strong heuristic of program improvement with use of search in order to provide improvements over a synthesizer model.
 
 We also contribute the TraceEmbed architecture, which augments information on the execution of the reference program. We show that TraceEmbed decreases the generalization and exact match error compared to existing work of program repair, and can be a useful component as part of SED.
